Cost-aware Joint Caching and Forwarding in Networks with Heterogeneous Cache Resources

Caching is crucial for enabling high-throughput networks for data intensive applications. Traditional caching technology relies on DRAM, as it can transfer data at a high rate. However, DRAM capacity is subject to contention by most system components and thus is very limited, implying that DRAM-only caches cannot scale to meet growing demand. Fortunately, persistent memory and flash storage technologies are rapidly evolving and can be utilized alongside DRAM to increase cache capacities. To do so without compromising network performance requires caching techniques adapted to the characteristics of these technologies. In this paper, we model the cache as a collection of storage blocks with different rate parameters and utilization costs. We introduce an optimization technique based on the drift-plus-penalty method and apply it in a framework which enables joint caching and forwarding. We show that it achieves an optimal trade-off between throughput and cache utilization costs in a virtual control plane. We then develop a corresponding practical policy in the data plane. Finally, through simulations in several settings, we demonstrate the superior performance of our proposed approach with respect to total user delay and cache utilization costs.

==> Body/S4_vip.tex <==
We adapt the VIP framework \cite{VIPoriginal} to develop our policy. We have three major reasons behind this decision. Firstly, this framework embeds the most critical parameter of a cache, the rate at which it can push objects into the network, directly into its analysis of network dynamics. Furthermore, it also ties caching with forwarding, which facilitates the design of a joint policy that can drive requests toward caching nodes while avoiding congestion in the network. Finally, the analysis of the framework is based on the {\it Lyapunov drift} technique, which allows us to formulate the trade-off between the queue backlog growth in the network and cache utilization costs through an approach called {\it drift-plus-penalty}.

\subsection{Framework Description}
\label{subsec:vipdynamics}

In the VIP framework, user demand for objects is measured using \textit{virtual interest packets} (VIPs), which are tracked in a {\it virtual} control plane separate from request and data delivery in the data plane.
%In the virtual plane, all request arrival and data delivery mechanisms are expressed at the object level.
Time in this plane is represented in slots of length 1 indexed as $t =  1,2, ...$ where time slot $t$ refers to the time interval $[t,t+1)$.
Each node $\nin$ keeps a separate counter $V^k_n(t)$ for each object $\kin$, which are all set to 0 at the beginning of time slot $t = 1$, with $V^k_n(t) = 0$ for all $t \geq 1$ if $n = \mc{S}(k)$. These are called {\it VIP counts} and represent the queue backlog for interests.
When a request for object $k$ enters the network at node $n$, the corresponding counter $V^k_n(t)$ is incremented. The number of requests for object $k$ that enter the network at node $n$ during slot $t$ is denoted as $A^k_n(t)$ and the external {\it arrival rate} of VIPs at node $n$ for object $k$ is $\lambda^k_n \triangleq \lim_{t \rightarrow \infty} \frac{1}{t}\sum^t_{\tau = 1} A^k_n(\tau)$.
Each time slot, nodes communicate their VIP counts and forward VIPs to their neighbors according to decisions made by a virtual plane algorithm. The allocated transmission rate of VIPs for object $k$ over link $(a,b)$ during slot $t$ is denoted as $\mu^k_{ab}(t)$. VIPs for an object $k$, after being forwarded through the virtual plane, are removed at either $\mc{S}(k)$ or nodes that cache $k$. Note that, in the data plane, the communication of VIPs can be handled with a single message of negligible size at each slot.
We define the {\it cache state} for object $k$ at node $n$ in tier $j$ during slot $t$ as $s^k_{n_j}(t) \in \{0,1\}$, where $s^k_{n_j}(t) = 1$ if the object is cached and $s^k_{n_j}(t) = 0$ otherwise, with $s^k_{n_j}(1) = 0, \; \forall \nin,\kin$.
A tier $j$ at node $n$ has {\it readout rate} $r_{n_j}$, meaning it can produce $r_{n_j}$ copies of each object it caches per time slot independent of other objects and tiers. We assume the cache tiers in the set are numbered in descending order of their readout rates, i.e. $r_{n_1} \geq r_{n_2} \geq \cdots$.

\subsection{Virtual Control Plane Algorithm}
\label{subsec:vipalgo}

We now describe our distributed joint caching and forwarding algorithm for the virtual plane in terms of the definitions above.
\begin{algorithm}[Caching and Forwarding in the Virtual Plane]
At the beginning of each time slot $t$, at each node $n$, observe VIP counts $(V^k_n(t))_{\kin, \nin}$, then perform forwarding and caching in the virtual plane as follows. \\
{\bf Caching:} At each node $\nin$, choose $s^k_{n_j}(t)$ for each data object $\kin$ and cache tier $\jin$ to
\begin{align}
    \text{maximize}
        & \quad \sum\limits_{\kin} \sum\limits_{\jin} b^k_{n_j}(t) s^k_{n_j}(t) \label{eq:gap_obj} \\
    \text{subject to}
        & \quad \sum\limits_{\kin} s^k_{n_j}(t) \leq L_{n_j}, \; \jin \label{eq:gap_const1} \\
        & \quad \sum\limits_{\jin} s^k_{n_j}(t) \leq 1, \; \kin \label{eq:gap_const2} \\
        & \quad s^k_{n_j}(t) \in \{0, 1\}, \; \kin, \; \jin \label{eq:gap_const3}
\end{align}
where,
\begin{equation}
    b^k_{n_j}(t) \triangleq \left\{ \begin{array}{ll}
        r_{n_j} V^k_n(t) - \omega c^a_{n_j}, & \text{if} \; s^k_{n_j}(t-1) = 0 \\
        r_{n_j} V^k_n(t) + \omega c^e_{n_j}, & \text{if} \; s^k_{n_j}(t-1) = 1
    \end{array} \right.
\label{eq:gap_benefits}
\end{equation}
and $\omega \geq 0$ is the importance weight of the penalty function defined as
\begin{equation}
    p^k_{n_j}(t) = 
    \left\{ \begin{array}{ll}
        c^a_{n_j}, & \text{if} \; s^k_{n_j}(t) - s^k_{n_j}(t-1) = 1 \\
        c^e_{n_j}, & \text{if} \; s^k_{n_j}(t) - s^k_{n_j}(t-1) = -1 \\
       0, & \text{otherwise}
   \end{array} \right.
\label{eq:pen}
\end{equation}
{\bf Forwarding:} Let $\mc{L}^k$ be the set of links which are allowed to transmit VIPs of object k, determined by a routing policy. For each data object $\kin$ and each link $\abin^k$, choose
    \begin{equation}
        \mu^k_{ab}(t) =
        \left\{ \begin{array}{ll}
            C_{ba}, & \text{if} \; k = k^*_{ab}(t) \; \text{and} \; W^k_{ab}(t) > 0 \\
            0, & \text{otherwise}
        \end{array} \right.
    \label{eq:mul_flowchoice}
    \end{equation}
where,
    \begin{equation}
    \begin{split}
        W^k_{ab}(t) & \triangleq V^k_a(t) - V^k_b(t), \\
        k^*_{ab}(t) & \triangleq \argmax\limits_{\{k: \abin^k\}} W^k_{ab}(t),
        %W^*_{ab}(t) & \triangleq \bigg( W^{k^*_{ab}(t)}_{ab}(t) \bigg)^+ ,
    \end{split}
    \label{eq:mul_fwddefs}
    \end{equation}
%where $W^k_{ab}(t)$ is the queue backlog differential \cite{tassiulas1990stability} of object $k$ on link $(a,b)$ at time $t$. \\
{\bf Queue Evolution:} Update VIP counts according to
\begin{equation}
\begin{split}
    V^k_n(t+1) \leq & \Bigg(\Big(V^k_n(t) - \sum\limits_{\bin}\mu^k_{nb}(t)\Big)^+ + A^k_n(t) \\ 
    & + \sum\limits_{\ain}\mu^k_{an}(t) - \sum\limits_{\jin} r_{n_j} s^k_{n_j}(t) \Bigg)^+    
\end{split}
\label{eq:evo}
\end{equation}
where $(x)^+ \triangleq \max(x,0)$.
\label{alg:mul_pen}
\end{algorithm}
The caching subproblem of Algorithm~\ref{alg:mul_pen} ensures an optimal placement of objects across cache tiers with respect to both the value of objects and the costs of admissions and replacements.
The importance weight $\omega$ acts as a control parameter allowing us to decide how much we value each side of this trade-off.
The last term in \eqref{eq:evo} represents VIPs removed via caching and lets us model the impact of the rate at which caches can satisfy requests, which directly affects network capacity and performance.
The penalty function \eqref{eq:pen} gets its name from the drift-plus-penalty approach and unifies the representation of cache utilization costs. Throughout the rest of the paper, we use the term {\it penalty} in reference to this function, in order to discern it from constants $c^a_{n_j}$ and $c^e_{n_j}$.

\subsection{Trade-off Optimality Analysis}
\label{subsec:vipanalysis}

We now provide an optimality analysis of our algorithm, which consists of two steps: (i) defining the capacity region of the network and (ii) showing the optimal trade-off between queue backlog reduction and total cache utilization cost.

\subsubsection{Capacity Region}
\label{subsubsec:vipcapacity}

As stated previously, our analysis of network queues in the virtual plane is based on the Lyapunov drift technique, which allows us to show that our algorithm can stabilize all network queues without a-priori knowledge of arrival rates. However, to show this property of the algorithm, a {\it capacity region} of the network with respect to arrival rates, for which there exists some feasible policy that can make all network queues rate stable, must first be defined \cite{neelybook}. A capacity region for the VIP network with single-tier caches is defined in \cite{VIPoriginal}. We now outline how this region is impacted by the inclusion of multiple tiers of cache.

\begin{theorem}[Capacity Region] The VIP capacity region $\Lambda$ of the network $\mc{G} = (\mc{N},\mc{L})$, is the set $\Lambda$ consisting of all VIP arrival rates $\boldsymbol{\lambda} = (\lambda^k_n)_{\kin,\nin}$ such that the following holds
\begin{equation}
\begin{split}
    \lambda^k_n \leq \sum\limits_{\bin} f^k_{nb} & - \sum\limits_{\ain} f^k_{an} + \sum\limits_{\jin} r_{n_j} \betasumind, \\
    & \forall \nin, \; \kin, \; n \not = \mc{S}(k)
\label{eq:flowcaching}
\end{split}
\end{equation}
\begin{equation}
    0 \leq \beta_{n,i} \leq 1, \quad i = 1,\cdots,\sigma, \quad \nin
\label{eq:prob}
\end{equation}
\begin{equation}
    \betasum = 1, \quad \forall \nin
\label{eq:probsum}
\end{equation}
where $f^k_{ab} = \sum^{t}_{\tau=1} F^k_{ab}(\tau)/t$ denotes the time average VIP flow for object $k$ over link $(a,b)$ and $F^k_{ab}(t)$ is the number of VIPs of $k$ transmitted over $(a,b)$ during slot $t$ and satisfying the following for all $t \geq 1$.
\begin{equation}
    F^k_{ab}(t) \geq 0, F^k_{nn}(t) = 0, F^k_{\mc{S}(k)n}(t) = 0, \; \forall a,b,n \in \mc{N}, \kin,
\end{equation}
\begin{equation}
    F^k_{ab}(t) = 0, \; \forall a,b \in \mc{N}, \kin, (a,b) \not \in \mc{L}^k
\end{equation}
\begin{equation}
    F^k_{ab}(t) \leq C_{ba}, \; \forall \abin
\end{equation}
$\mathcal{B}_{n,i}$ denotes the $i$-th one among $\sigma$ total number of possible cache placement sets at node $n$, and $\beta_{n,i}$ represents the fraction of time that objects are placed at $n$ according to $\mc{B}_{n,i}$. The elements of set $\mc{B}_{n,i}$ are pairs in the form of $(k,j)$, such that if $(k,j) \in \mc{B}_{n,i}$, object $k$ is cached in tier $j$.
\begin{proof}
Please see Appendix \ref{app:stability}.
\end{proof}
\label{thm:stability}
\end{theorem}

\begin{comment}
\begin{figure}[!t]
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{Figures/vip-queue-sum-3.pdf}
    \caption{Queue backlog}
    \label{fig:virtual_vips}
  \end{subfigure}
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{Figures/penalty-sum-3.pdf}
    \caption{Penalty}
    \label{fig:virtual_pens}
  \end{subfigure}
  \caption{Evolution of total VIP queue backlog and total penalty over time in the virtual plane (Abilene topology of Figure~\ref{fig:tops}, $\abs{\mc{N}}=1000$, $\sum_{\kin}\lambda^k_n=10$, $\omega = 3$).}
  \label{fig:overtime}
\end{figure}
\end{comment}

\subsubsection{Backlog-Penalty Bound Tradeoff}
\label{subsubsec:tradeoff}

We now show that our algorithm can achieve the optimal trade-off between queue backlog growth and cache utilization costs, using the drift-plus-penalty approach.
%In this context, penalty refers to the value of the function \eqref{eq:pen}. Throughout the rest of the paper, we use the term penalty to distinguish 
%We now use the {\it drift-plus-penalty} approach \cite{neelybook} to show that our algorithm can achieve the optimal trade-off between queue backlog and penalty bounds.
We assume that request arrival processes are mutually independent for all nodes and objects, and are i.i.d. with respect to time slots. We also assume that there is a finite value $A^k_{n,max}$ such that $A^k_n(t) \leq A^k_{n,max}$ for all $n$, $k$ and $t$.

\begin{theorem}[Throughput and Penalty Bounds] Given the VIP arrival rate vector $\boldsymbol{\lambda} = (\lambda^k_n)_{\kin,\nin} \in int(\Lambda)$, if there exists $\boldsymbol{\epsilon} = (\epsilon^k_n)_{\nin, \kin} \succ \mathbf{0}$ such that $\boldsymbol{\lambda} + \boldsymbol{\epsilon} \in \Lambda$, then the network of VIP queues under Algorithm \ref{alg:mul_pen} satisfies
\begin{equation}
    \lim\limits_{T \rightarrow \infty} \frac{1}{T} \sum\limits^{T-1}_{t=0} \sum\limits_{\nin, \kin} \mathbbm{E}[V^k_n(t)] \leq \frac{NB}{\epsilon} + \frac{\omega}{2\epsilon} \minpen
\label{eq:vipbound}
\end{equation}
\begin{equation}
    \lim\limits_{T \rightarrow \infty} \frac{1}{T}\sum\limits^{T-1}_{t=0} \mathbbm{E}[p(t)] \leq \frac{2NB}{\omega} + \minpen
\label{eq:penbound}
\end{equation}
where $\epsilon \triangleq \textstyle \min_{\nin,\kin} \epsilon^k_n$, $p(t) = \sum_{\kin, \nin, \jin} p^k_{n_j}(t)$ is the total penalty accumulated across the network at slot $t$, $\Psi(\boldsymbol{\lambda})$ is the minimum long term average total penalty achievable by any feasible policy that makes all queues rate stable \cite{neelybook} and,
\begin{align}
    B \triangleq \frac{1}{2N} \sum_{\nin} & \bigg(\big(\textstyle \sum_{\bin}C_{nb}\big)^2 + 2\big(\textstyle \sum_{\bin}C_{nb}\big)\abs{\mc{K}}r_{n_1} \\ 
    & + \big(\textstyle \sum_{\kin}A^k_{n,max} + \textstyle \sum_{\ain}C_{an} + \abs{\mc{K}}r_{n_1}\big)^2 \bigg)
\end{align}
%where $\epsilon \triangleq \min\limits_{\nin,\kin} \epsilon^k_n$, $B \triangleq \frac{1}{2N} \sum_{\nin} \big((\mu^{out}_{n,max})^2 + 2\mu^{out}_{n,max}r_{n,max} + (A_{n,max} + \mu^{in}_{n,max} + r_{n,max})^2 \big)$, $\mu^{out}_{n,max} \triangleq \sum_{\bin}C_{nb}/z$, $\mu^{in}_{n,max} \triangleq \sum_{\ain}C_{an}/z$, $A_{n,max} \triangleq \sum_{\kin}A^k_{n,max}$, and $r_{n,max} \triangleq Kr_{n_1}$ where $r_{n_1} \geq r_{n_j}, \forall \jin$.
\begin{proof}
Please see Appendix \ref{app:dpp}.
\end{proof}
\label{thm:dpp}
\end{theorem}

Theorem~\ref{thm:dpp} demonstrates the adjustable trade-off between queue backlogs and penalties: we can set $\omega$ arbitrarily large to push the time average penalty close to the minimum $\Psi(\boldsymbol{\lambda})$ at the cost of significantly increasing the average queue backlog and vice-versa. Figure~\ref{fig:avgs} visualizes this dynamic in the virtual plane.

\begin{figure}[!t]
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{Figures/vip-queue-avg.pdf}
    \caption{Sum of VIP counts}
    \label{fig:virtual_vip_avg}
  \end{subfigure}
  \begin{subfigure}[b]{0.215\textwidth}
    \includegraphics[width=\textwidth]{Figures/penalty-avg.pdf}
    \caption{Sum of penalties}
    \label{fig:virtual_pen_avg}
  \end{subfigure}
  \caption{Long-term average of total VIP queue backlog and total penalty in the virtual plane (Abilene topology of Figure~\ref{fig:tops}, $\abs{\mc{N}}=1000$, $\sum_{\kin}\lambda^k_n=10$).}
  \label{fig:avgs}
\end{figure}

\subsubsection{Optimal Solution to the Caching Subproblem}
\label{subsubsec:solution}

We have shown through Theorem~\ref{thm:dpp} that Algorithm~\ref{alg:mul_pen} optimizes the backlog-penalty trade-off. However, for Theorem~\ref{thm:dpp} to hold we must solve the caching subproblem defined by \eqref{eq:gap_obj}--\eqref{eq:gap_const3} exactly.
While this problem appears in the form of a generalized assignment problem (GAP), which is known to be NP-hard, we can show that it is in fact a rectangular assignment problem (RAP) by using a simple transformation of variables, which we present in the following lemma.
%This problem appears to be in the form of a generalized assignment problem (GAP), which is known to be NP-hard.
%However, using a transformation of variables, we can rewrite it in the form of a rectangular linear assignment problem (RLAP), which can be solved exactly in polynomial time using a modification of the Jonker-Volgenant algorithm \cite{volgenant1996linear,crouse2016implementing}. This is possible for our model since we assume that all data objects in the network have the same size. The following lemma describes this transformation of variables.

\begin{lemma}
Let $i$ be an integer in the set of integers $\mc{I}_n = \{1, 2, ..., \\  \sum_{\jin} L_{n_j}\}$. Let $b^k_{n_j}(t) = b^k_{n_i}(t)$ and $s^k_{n_j}(t) = s^k_{n_i}(t)$ if $i \in \mc{I}_{n_j} = \{1 + \sum^{j - 1}_{\ell = 1} L_{n_\ell}, ..., \sum^{j}_{\ell = 1} L_{n_\ell}\}$. Then, a solution to the following problem gives an equivalent solution to the problem defined by \eqref{eq:gap_obj}--\eqref{eq:gap_const3}.
\begin{align}
    \text{maximize}
        & \quad \sum\limits_{\kin} \sum\limits_{\iin} b^k_{n_i}(t) s^k_{n_i}(t) \label{eq:lsap_obj}\\
    \text{subject to} 
        & \quad \sum\limits_{\kin} s^k_{n_i}(t) \leq 1, \; \iin \label{eq:lsap_const1} \\
        & \quad \sum\limits_{\iin} s^k_{n_i}(t) \leq 1, \; \kin \label{eq:lsap_const2} \\
        & \quad s^k_{n_i}(t) \in \{0, 1\}, \; \kin, \; \iin \label{eq:lsap_const3}
\end{align}
\begin{proof}
    Since $|\mc{I}_{n_j}| = L_{n_j}$, $s^k_{n_j}(t) = 1$ can hold for at most $L_{n_j}$ objects. Therefore, \eqref{eq:lsap_const1} is equivalent to \eqref{eq:gap_const1}. Furthermore, since $s^k_{n_i} = 1$ can hold for at most one $i \in \mc{I}_n$, \eqref{eq:lsap_const2} is equivalent to \eqref{eq:gap_const2}.
\end{proof}
\label{lem:rap}
\end{lemma}

The problem defined by \eqref{eq:lsap_obj}-\eqref{eq:lsap_const3} has the form of a RAP and can be solved exactly in polynomial time using a modified Jonker-Volgenant algorithm \cite{volgenant1996linear,crouse2016implementing}. Since \eqref{eq:lsap_const1} is an inequality, in cases where $b^k_{n_i}(t) < 0$ for some $i \in \mc{I}_n$, we can obtain the optimal solution by treating \eqref{eq:lsap_const1} as an equality, then setting $s^k_{n_i}(t) = 0$ for all $i$ such that $b^k_{n_i}(t) < 0$.
%Note that, while the problem presented in Lemma~\ref{lem:rap} is in the form of a RLAP, the constraint in \eqref{eq:lsap_const1} is an inequality.
%This means that, in a case where $b^k_{n_i}(t) < 0$ for some $i \in \mc{I}_n$, the problem in Lemma~\ref{lem:rap} has a larger set of feasible solutions than a RLAP. Fortunately, this difference is trivial to manage, as the optimal solution for such a case can be obtained by solving the problem treating \eqref{eq:lsap_const1} as an equality, then setting $s^k_{n_i}(t) = 0$ for all $i$ such that $b^k_{n_i}(t) < 0$.

It is important to point out that the equivalence of \eqref{eq:gap_obj}--\eqref{eq:gap_const3} to \eqref{eq:lsap_obj}-\eqref{eq:lsap_const3} is due to the assumption in our model that all objects have the same size. However, the problem formulated by \eqref{eq:gap_obj}--\eqref{eq:gap_const3} can be generalized to a model where objects have different sizes, in which case it would indeed be a GAP. Polynomial time methods that can approximate a solution to the GAP exist \cite{shmoys1993approximation,fleischer2006tight,feige2006approximation}. While the results of Theorem~\ref{thm:dpp} would not hold for an approximate solution, it may be possible to show that they would hold for arrival rates in the interior of a subset of $\Lambda$, the bounds of which depend on the factor of approximation.
%It is important to point out that, while we assumed all objects to be of the same size in our model, the problem formulated by \eqref{eq:gap_obj}--\eqref{eq:gap_const3} can be generalized to a model where objects have different sizes. In that case, we would need to develop an approximate solution to the initial GAP. Methods to do so that can guarantee different factors of approximation exist \cite{shmoys1993approximation,fleischer2006tight,feige2006approximation}. However, with an approximate solution, the results of Theorem~\ref{thm:dpp} will not hold, though it can be shown that the queues can still be stabilized given that the arrival rates are in the interior of a subset of $\Lambda$.

\begin{figure}[!t]
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{Figures/abilene.pdf}
    \caption{Abilene Network}
    \label{fig:tops_ab}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.20\textwidth}
    \includegraphics[width=\textwidth]{Figures/geant.pdf}
    \caption{GEANT Network }
    \label{fig:tops_geant}
  \end{subfigure}
  \caption{Network Topologies}
  \label{fig:tops}
\end{figure}

\subsection{Practical Policy for the Data Plane}
\label{subsec:practical}

When node $n$ receives a new request for object $k$ in the data plane, it first checks to see if $k$ is found in any of its cache tiers. If so, the request is satisfied by retrieving a copy of the object from that tier. If not, the request is forwarded to a neighboring node $b$ for which $(n,b) \in \mc{L}$. When data object $k$ arrives at a node which does not already cache $k$, that node makes a caching decision that includes whether to admit the object, which tier to admit it in if so, and which object already cached in that tier to replace if any. We now describe how these caching and forwarding decisions are made in the data plane. Note that the theoretical results demonstrated for the policies in the virtual plane do not carry over to the data plane. Rather, our goal in the data plane is making forwarding and caching decisions by using the joint policy in the virtual plane as a guideline.

\subsubsection{Caching in the Data Plane}
Implementing a caching policy in the data plane based on Algorithm~\ref{alg:mul_pen} requires significant adjustments due to gaps between the assumptions of the virtual control plane and the constraints of the data plane. Firstly, in the virtual plane, it is assumed that once the cache state variables are set, the contents of the cache are immediately updated. However, in the data plane, the instance when an object can be cached at a node will differ from the virtual control plane time slot when the decision to cache that object was made. Secondly, as mentioned in \cite{VIPoriginal}, since VIPs for an object are drained immediately after the object is cached, Algorithm~\ref{alg:mul_pen} leads to frequent shifts in cache distribution. While the drift-plus-penalty approach allows us to better manage this behavior, it faces a different issue in balancing the constant cost parameters that contribute to penalties against the large swings in VIP counts that can happen within a time slot. Having highlighted these gaps, we present a practical caching policy in the data plane that is based on the VIP flows established by Algorithm~\ref{alg:mul_pen}.

We adopt the {\it cache score} metric devised in the stable caching algorithm presented in \cite{VIPoriginal}. Let $v^k_{ab}(t) \leq \mu^k_{ab}(t)$ be the actual number of VIPs for object $k$ transmitted over link $(a,b)$ during slot $t$ and let $T$ be the size of a sliding window. The cache score for object $k$ at node $n$ at time $t$ is defined as the average number of VIPs for object $k$ received by node $n$ over a sliding window of $T$ time slots prior to time slot $t$, expressed as follows.
\begin{equation}
    CS^k_n(t) = \frac{1}{T} \sum^t_{\tau = t - T + 1} \sum_{(a,n) \in \mc{L}^k} v^k_{an}(\tau) = \sum_{(a,n) \in \mc{L}^k} \widebar{v}^k_{an}(t)
    \label{eq:cache_scores}
\end{equation}
We then define the {\it cache benefit} metric, which balances the cache score against utilization costs, as follows.
\begin{equation}
    CB^k_{n_j}(t) = \begin{cases}
        \begin{array}{l}
             r_{n_j}(CS^k_n(t) - CS^{k'}_n(t)) - \omega(c^a_{n_j} + c^e_{n_j}), \text{if} \, j \, \text{is full} \\
             r_{n_j} CS^k_n(t) - \omega c^a_{n_j}, \; \text{otherwise}
        \end{array}
    \end{cases} 
    \label{eq:cache_benefit}
\end{equation}
where $k'_{n_j} = \argmin_{\{k \in \mc{K}_{n_j}\}} CS^k_n(t)$ with $\mc{K}_{n_j}$ denoting the set of currently cached objects across all tiers at node $n$ at a given time.

When a data object $k \not \in \mc{K}_{n_j}$ arrives at node $n$ during a time interval $[t,t)$, the caching policy first determine the cache tier which offers the highest cache benefit, i.e. $j^* = \argmax_{\{ \jin \}} CB^k_{n_j}(t)$. If $CB^k_{n_{j^*}}(t) > 0$, the object is admitted to tier $j^*$. If tier $j^*$ is full, object $k$ replaces object $k'_{n_j}$ defined above. If $j^*$ has free capacity, no replacements occur. We repeat this process as long as there are replacements, treating any replaced object as if it is a new data object arrival to see if there is a positive benefit to migrating it to a different cache tier.

\subsubsection{Forwarding in the Data Plane}
A request for object $k \not \in K_{n_j}$ that arrives at node $n$ is forwarded to node
\begin{equation}
    b^k_n(t) = \argmax_{\{ b:(n,b) \in \mc{L}^k \}} \frac{1}{T} \sum\limits^t_{t'=t-T+1} v^k_{ab}(t)
    \label{eq:dataplanefwd}
\end{equation}
This policy tries to forward objects on links that are most profitable according to the flow pattern of VIPs in the virtual plane. As the process of forwarding VIPs in the virtual plane is periodic, the sliding window is used to represent the time-average behavior of that process. This establishes a measurement the forwarding policy in the data plane can use to follow the patterns in the virtual plane.

Note that the policies we describe above are expressed only in object level terms. In an actual implementation, data objects will be made up of several {\it chunks}. Our policies would employ the following two principles at the chunk level. If a data object is admitted to a cache tier, all its chunks must be admitted to the same tier and if a data object is evicted from a cache tier, all its chunks must be evicted from that tier. The forwarding decision described in \eqref{eq:dataplanefwd} is made when a request for the first chunk of object $k$ arrives at node $n$: all requests for subsequent chunks of $k$ are forwarded to the same node.

==> Body/S7_limitations.tex <==
In the model and policies we propose, there are certain directions for future improvement.
Firstly, given the data delivery mechanics of our model, our policy can run into issues where an object that has been previously cached in a slower tier at a node sees a significant increase in demand, but cannot be moved to a faster tier in that node since requests for it are never forwarded upstream. To work around this problem, we could devise {\it proactive migration} schemes, where objects can be moved between cache tiers independently of request arrival and data delivery processes. An example of a practical approach is to periodically poll the placement of objects across all tiers and carry out the most beneficial migrations that can be completed in a reasonable time frame.
Secondly, the assumption in the VIP framework that the readout rate of a cache tier is independent for each object does not translate well to the data plane since cache devices have a shared bandwidth. A solution to amend this gap is to express the readout rates as dynamic parameters which are tied together by a total rate constraint. This solution presents another problem dimension in the optimal selection of these dynamic parameters. However, that dimension can also be approached in the virtual plane using the backpressure-based tools provided by the framework.

==> Body/old_intro.tex <==
One of the core components enabling high performance information-centric networking (ICN) architectures is caching. Caching is intrinsic to the ICN paradigm and has great impact on the overall network performance. The two main parameters of a cache that impact network performance are its speed and capacity. The traditional cache device is DRAM, despite its small capacity, since it has access speeds that can match network link speeds. However, as the amount of data carried by networks increases, the small capacity of DRAM becomes an obstacle in scaling network performance via caching.
Fortunately, permanent storage technologies are advancing rapidly and it may soon be possible to use these devices along with DRAM to enable larger caches. Designs that address this {\it vertical} expansion of caches already exist in the literature, and given the potential performance improvements with the next evolution of the PCIe and NVMe standards, as well as technologies like SPDK \cite{yang2017spdk}, it is safe to say the wider implementation of ICN routers with large multi-layered caches is around the corner.

While disk storage today offers large capacities at small upfront costs, utilizing them as short-term caches may introduce significant operational costs, as they consume significant amounts of power and their reliability reduces over time with use. Therefore, the performance benefits and operational costs of utilizing these devices must be carefully balanced in order to build sustainable high performance networks. One of the major factors in this balancing act is the cache admission and replacement strategy.

In this paper, we propose a caching strategy that optimally utilizes multiple types of memory and storage elements with different characteristics. The goal of our strategy is to find the optimal trade-off between the performance gained via caching and the costs incurred by utilizing caches. We develop our caching strategy jointly with forwarding, adopting the VIP framework presented in \cite{VIPoriginal} to do so. In the VIP framework, user demand for objects is the main metric guiding caching and forwarding decisions, which is an appropriate measure for our goals. Furthermore, we believe the effectiveness of our caching strategy will be amplified in combination with VIP's innate ability to drive requests toward caching points in the network while avoiding congestion. The contributions of this paper can be summarized as follows:

\begin{itemize}
    \item A caching model that considers multiple tiers of cache with different performance parameters, as well as the costs of utilizing these cache tiers,
    \item An extension of the VIP framework of \cite{VIPoriginal}, in view of our proposed caching model,
    \item A distributed joint caching and forwarding algorithm emerging from this extended framework which minimizes a combined objective of queue growth bound and caching costs.
\end{itemize}

%The rest of this paper is structured as follows. In Section 2, we go over related work in the ICN literature, as well as other literature where hybrid memory-storage systems take focus. In Section 3, we present formal descriptions of our network and caching models. In Section 4, we give a brief overview of the VIP framework and its dynamics in consideration of our caching model. Because the VIP framework employs a virtual control plane on top of the actual plane where packets flow, we first introduce, in Section 5, our joint caching and forwarding algorithm as it operates in the virtual plane. We then follow this up in Section 6 with how the virtual plane algorithm guides forwarding and caching in the actual plane. In Section 7, we evaluate the performance of our proposed strategy numerically, comparing it to several baselines, some of which we extend to our multi-tiered caching model.

%In order to characterize all tiers of cache with a shared set of parameters, while staying as agnostic to use cases as possible, we consider the following for each tier in our model: (i) their read and write speeds, (ii) their energy consumption and (iii) their endurance, which refers to the impact of writes on their lifetime. While endurance in this context is mostly irrelevant for DRAM, it is of critical importance for the health of storage devices. Energy consumption, on the other hand, is a cost applicable to any type of memory or storage element and makes up the bulk of operational costs in any computer system. Because object replacements across caches can occur frequently, we must take care not to overuse these devices when benefits of doing so are minimal. These parameters establish the basis with which we measure the benefits and costs of placing and migrating objects across cache tiers.

==> Body/old_related.tex <==
The challenge of optimal data placement in multi-layered storage architectures have long been a focus of research in systems like data centers or cloud storage platforms. In these contexts, vast amounts of data need to be kept in storage for long periods of time. To provide low latency access to popular portions of this data, techniques that use SSDs as caches for HDDs are widely adopted \cite{niu2018hybrid}. Novel techniques aimed at modern enterprise storage systems where all storage elements are SSDs (all-flash) have also been developed \cite{yang2017autotiering}. Most recently, reinforcement learning was applied to the data placement problem in hybrid storage systems to provide an adaptive and continuously improving solution \cite{singh2022sibyl}.

The optimal data placement challenge for the in-network caching context may appear similar. However, the crucial difference is that in-network caching places cache devices directly on the forwarding path of requests and data. Therefore, bottlenecks in the caching system lead to compounding network-wide performance issues. As such, in-network caching has much stricter demands from storage systems and lower tolerance for overheads.
Still, the feasibility of devices beyond DRAM as caches in a data delivery network context have been explored, primarily for the information-centric networking (ICN) paradigm.
%The initial perspective on using devices like SSDs for caching in ICN architectures was somewhat skeptical \cite{perino2011reality}, as storage technologies improved, system designs that make use of them for terabyte-scale ICN caches appeared.
While SSDs were initially seen as either too costly or not performant enough for ICN \cite{perino2011reality}, as storage technologies improved, system designs that make use of them for terabyte-scale ICN caches appeared.
%In \cite{rossini2014multi}, it was observed that moving the SSD bottleneck from access latency to external transfer rate could lead to an order of magnitude increase in performance. Based on this observation, the authors designed a two-layer cache structure with a large SSD layer masked behind a fast DRAM layer.
In \cite{rossini2014multi}, the authors observed that moving the SSD bottleneck from access latency to external transfer rate could lead to a significant gain in performance, and designed a two-layer cache structure with a large SSD layer masked behind a fast DRAM layer.
They made use of common ICN request patterns as a predictor for prefetching data from the SSD cache into the DRAM cache, using LRU as the replacement policy. A follow-up work \cite{mansilha2015hierarchical} used this design in a high-speed router prototype which achieved more than 10Gbps throughput. Another design was proposed in \cite{so2014toward}, where block device I/O was separated from forwarding paths by sending packets to a dedicated caching process, allowing forwarding to continue operating at line-rate while enabling terabyte-scale caches. However, SSD-based caches have yet to see wider adoption in modern ICN prototypes. In \cite{shi2020ndn}, where a high-throughput software-defined forwarder for Named Data Networking (NDN) was introduced, caching in persistent memory or NVMe disk storage was stated as a future direction and the necessity for novel caching algorithms accounting for the varying device characteristics in a multi-tiered cache was outlined. A recent experimental study for a high performance NDN-based data delivery system using this forwarder featured nodes with DRAM-only caches of 20~GB capacity \cite{wu2022ndise}.

%A significant roadblock in the way of this paradigm shift is the lack of caching policies that address the optimal data placement problem within the constraints of a networking context. \com{talk about policies?}

==> overview.tex <==
\begin{enumerate}
    \item {\bf Introduction}
        \begin{itemize}
            \item Motivation: "Caches need to operate at line rate and SSDs are slow -> SSD technology has improved significantly and continues to -> we can use them but need to do so carefully as to optimize resource use -> current strategies can't handle this
        \end{itemize}
    \item {\bf Related Background}
        \begin{itemize}
            \item Implementations of SSD-based content stores in ICN routers
            \item Limitations outlined in the NDN-DPDK and N-DISE papers
            \item Adaptable strategies and VIP
            \item \com{Relevant discussions of cache placement in tiered caches from outside ICN literature?}
        \end{itemize}
    \item {\bf System Model}
        \begin{itemize}
            \item Define {\it data, data object, request, network graph, link, link capacity, request-data traversal, cache tier, cache capacity, cache exclusivity, migration, admission and eviction costs}
        \end{itemize}
    \item {\bf Extensions}
        \begin{itemize}
            \item (LCE)+LRU/+UNIF as examples of "naive" extensions that won't do well to illustrate why multi-tier requires specialized approach
            \item A class of algorithms where there's a bounded (and ideally time-averaged?) metric that can be used to determine benefit of caching to weigh against cost. LFU is the simplest example for this. VIP is another where the technique yields optimal trade-off in the virtual plane.
        \end{itemize}
    \item {\bf VIP Extension}
        \begin{itemize}
            \item <Most significant contribution> Drift-plus-penalty trade-off optimizaiton for VIP (MVIP)
            \item \com{"Naive" extension of single-tier VIP just as in LFU (SVIP)?}
        \end{itemize}
    \item {\bf Numerical Results}
        \begin{itemize}
            \item Setting and test case descriptions \com{need to mention the routing somewhere, maybe here?}
            \item Impact of the slower cache's size and why naive extensions of widely used algorithms won't work
            \item Delay vs request rate for LFU, SVIP and MVIP
            \item Delay vs penalty for LFU, SVIP and MVIP
        \end{itemize}
    \item {\bf Limitations and Challenges}
        \begin{itemize}
            \item Gap between system model and real systems
            \item Limitations of experiments
            \item Limitations of VIP, gap between virtual and actual planes
        \end{itemize}
    \item {\bf Conclusion and Future Directions}
\end{enumerate}
